Uniformly sampling random directed hypergraphs with fixed degrees

Many complex systems show non-pairwise interactions, which can be captured by hypergraphs. In this work, we propose an edge-swapping method to sample random directed hypergraphs with fixed vertex and hyperarc degrees, which can be applied to different classes of directed hypergraphs (containing self-loops, degenerate hyperarcs and/or multi-hyperarcs). We prove that this method indeed samples uniformly from the classes with self-loops and multi-hyperarcs, and that the method may not sample uniformly from classes without self-loops, or with self-loops and degenerate hyperarcs but without multi-hyperarcs. We present a partial result on the class with self-loops, but without degenerate hyperarcs or multi-hyperarcs.

==> proofs/uniformity_proofs.tex <==
\begin{proof}[Proof of Theorem \ref{thm:uniform_alldegrees}]
    Since $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,d,p})$ and $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,p})$ are aperiodic (Lemma \ref{lemma:aperiodic})
    and strongly connected (Lemmas \ref{lemma:stub_spd_connected} and \ref{lemma:stub_sp_connected}, respectively), random walks on $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,d,p})$ and $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,p})$ are ergodic. Since $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,d,p})$ and $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,p})$ is also regular (Lemma \ref{lemma:regular}), both have a unique uniform stationary distribution. 
\end{proof}

 \begin{proof}[Proof of Theorem \ref{thm:uniform_degrees(2,1)}]
    Since $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s})$ is aperiodic (Lemma \ref{lemma:aperiodic})
    and strongly connected for any degree sequence with $d_a^{\textnormal{t}}=2,d_a^{\textnormal{h}}=1$ (Lemma ...), random walks on $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s})$ are ergodic. Since $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s})$ is also regular (Lemma \ref{lemma:regular}), $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s})$ has a unique uniform stationary distribution for any degree sequence with $d_a^{\textnormal{t}}=2,d_a^{\textnormal{h}}=1$. 
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:notuniform}]
    By Lemma \ref{lemma:stub_sd_notconnected}, $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{s,p})$ is not strongly connected, for at least one degree sequence. By Lemma \ref{lemma:stub_many_notconnected}, $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{d,p})$, $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{d})$, $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{p})$ and $\mathcal{G}(\mathcal{H}^{\textnormal{stub}}_{})$ are not strongly connected, for at least one degree sequence. Therefore, these directed hypergraph spaces do not have a unique uniform stationary distribution, for at least one degree sequence. 
\end{proof}
